The Heterophilic Graph Learning Handbook: Benchmarks, Models, Theoretical Analysis, Applications and Challenges

Homophily principle, \ie{} nodes with the same labels or similar attributes are more likely to be connected, has been commonly believed to be the main reason for the superiority of Graph Neural Networks (GNNs) over traditional Neural Networks (NNs) on graph-structured data, especially on node-level tasks. However, recent work has identified a non-trivial set of datasets where GNN's performance compared to the NN's is not satisfactory. Heterophily, i.e. low homophily, has been considered the main cause of this empirical observation. People have begun to revisit and re-evaluate most existing graph models, including graph transformer and its variants, in the heterophily scenario across various kinds of graphs, e.g. heterogeneous graphs, temporal graphs and hypergraphs. Moreover, numerous graph-related applications are found to be closely related to the heterophily problem. In the past few years, considerable effort has been devoted to studying and addressing the heterophily issue. In this survey, we provide a comprehensive review of the latest progress on heterophilic graph learning, including an extensive summary of benchmark datasets and evaluation of homophily metrics on synthetic graphs, meticulous classification of the most updated supervised and unsupervised learning methods, thorough digestion of the theoretical analysis on homophily/heterophily, and broad exploration of the heterophily-related applications. Notably, through detailed experiments, we are the first to categorize benchmark heterophilic datasets into three sub-categories: malignant, benign and ambiguous heterophily. Malignant and ambiguous datasets are identified as the real challenging datasets to test the effectiveness of new models on the heterophily challenge. Finally, we propose several challenges and future directions for heterophilic graph representation learning.

==> applications.tex <==
\begin{figure*}[ht!]
\centering
%\resizebox*{!}{\dimexpr\textheight-4\baselineskip\relax}{
\resizebox{1.0\textwidth}{!}{
\begin{forest}
    for tree={%
        my node,
        l sep+=5pt,
        grow'=east,
        edge={gray, thick},
        parent anchor=east,
        child anchor=west,
        if n children=0{tier=last}{},
        edge path={
            \noexpand\path [draw, \forestoption{edge}] (!u.parent anchor) -- +(10pt,0) |- (.child anchor)\forestoption{edge label};
        },
        if={isodd(n_children())}{
            for children={
                if={equal(n,(n_children("!u")+1)/2)}{calign with current}{}
            }
        }{}
    }
    [\textbf{Heterophily-Related Applications}, draw=black
    [\textbf{Fraud/Anomaly/Bot Detection} \ref{sec:9.1}, draw=green, top color=green!10, bottom color=green!10
        [\textbf{Fraud Detection} \ref{sec:9.1.1}, draw=green, top color=green!20, bottom color=green!20
            [\textbf{Neighborhood Partitioning and Grouping}, draw=green, top color=green!20, bottom color=green!20
                [H$^2$-FDetector~\cite{shi2022h2}, draw=green]
                [GAGA~\cite{wang2023label}, draw=green]
                [DRAG~\cite{kim2023dynamic}, draw=green]
            ]
            [\textbf{Spectral-Based Methods}, draw=green, top color=green!30, bottom color=green!30
                [SEC-GFD~\cite{xu2023revisiting}, draw=green]
                [SplitGNN~\cite{wu2023splitgnn}, draw=green]
            ]
        ]
        [\textbf{Anomaly Detection} \ref{sec:9.1.2}, draw=green, top color=green!30, bottom color=green!30
            [\textbf{Graph Structure Augmentation}, draw=green, top color=green!30, bottom color=green!30
                [GHRN~\cite{gao2023addressing}, draw=green]
                [SparseGAD~\cite{gong2023beyond}, draw=green]
                [HedGe~\cite{zhang2024generation}, draw=green]
            ]
            [\textbf{Metric-Guided Detection}, draw=green, top color=green!30, bottom color=green!30
                [TAM~\cite{qiao2024truncated}, draw=green]
            ]
            [\textbf{GAD-Specific Information Propagation}, draw=green, top color=green!30, bottom color=green!30
                [GDN~\cite{gao2023alleviating}, draw=green]
            ]
        ]
        [\textbf{Bot Detection} \ref{sec:9.1.3}, draw=green, top color=green!40, bottom color=green!40
            [BothH~\cite{li2023multi}, draw=green]
            [HOVER~\cite{ashmore2023hover}, draw=green]
            [HOFA~\cite{ye2023hofa}, draw=green]
        ]
    ]
    [\textbf{Generative Models} \ref{sec:9.2}, draw=red, top color=red!10, bottom color=red!10
        [\textbf{Molecule Generation} \ref{sec:9.2.1}, draw=red, top color=red!20, bottom color=red!20
            [HTFlows~\cite{wang2024molecule}, draw=red]
        ]
        [\textbf{Scene Graph Generation} \ref{sec:9.2.2}, draw=red, top color=red!30, bottom color=red!30
            [HL-Net~\cite{lin2022hl}, draw=red]
            [KWGNN~\cite{chen2024kumaraswamy}, draw=red]
        ]
    ]
    [\textbf{Classification and Clustering Tasks} \ref{sec:9.3}, draw=blue, top color=blue!10, bottom color=blue!10
        [\textbf{Link Prediction} \ref{sec:9.3.1}, draw=blue, top color=blue!20, bottom color=blue!20
            [DisenLink~\cite{zhou2022link}, draw=blue]
            [GRAFF-LP~\cite{di2023understanding}, draw=blue]
        ]
        [\textbf{Graph Classification} \ref{sec:9.3.2}, draw=blue, top color=blue!30, bottom color=blue!30
            [IHGNN~\cite{ye2022incorporating}, draw=blue]
            [MGS~\cite{ding2023self}, draw=blue]
        ]
        [\textbf{Graph Clustering} \ref{sec:9.3.3}, draw=blue, top color=blue!40, bottom color=blue!40
            [DGCN~\cite{pmlr-v202-pan23b}, draw=blue]
            [HoLe~\cite{gu2023homophily}, draw=blue]
            [AHGFC~\cite{wen2024homophily}, draw=blue]
        ]
    ]
    [\textbf{Recommender System} \ref{sec:9.4}, draw=yellow, top color=yellow!10, bottom color=yellow!10
        [SHaRe~\cite{jiang2024challenging}, draw=yellow]
    ]
    [\textbf{Biomedical} \ref{sec:9.5}, draw=violet, top color=yellow!10, bottom color=yellow!10
        [\textbf{Combination Therapy} \ref{sec:9.5.1}, draw=violet, top color=violet!20, bottom color=violet!20
            [DCMGCN~\cite{chen2022drug}, draw=violet]
        ]
        [\textbf{Drug Repositioning} \ref{sec:9.5.2}, draw=violet, top color=violet!30, bottom color=violet!30
            [SLGCN~\cite{liu2024slgcn}, draw=violet]
        ]
        [\textbf{Drug Discovery} \ref{sec:9.5.3}, draw=violet, top color=violet!40, bottom color=violet!40
            [HTFlows~\cite{ye2022incorporating}, draw=violet]
        ]
    ]
    [\textbf{Knowledge Distillation} \ref{sec:9.6}, draw=orange, top color=orange!10, bottom color=orange!10
        [SA-MLP~\cite{chen2022sa}, draw=orange]
        [VQGraph~\cite{yang2024vqgraph}, draw=orange]
    ]
    [\textbf{Adversarial Attack and Robustness} \ref{sec:9.7}, draw=brown, top color=brown!10, bottom color=brown!10
        [\textbf{Graph Structure Augmentation} \ref{sec:9.7.1}, draw=brown, top color=brown!20, bottom color=brown!20
            [GNNGUARD~\cite{zhang2020gnnguard}, draw=brown]
            [LP4GLN~\cite{cheng2023label}, draw=brown]
            [LHS~\cite{qiu2023refining}, draw=brown]
        ]
        [\textbf{Robust Graph Filter and Network Architecture} \ref{sec:9.7.2}, draw=brown, top color=brown!30, bottom color=brown!30
            [EvenNet~\cite{lei2022evennet}, draw=brown]
            [NSPGNN~\cite{zhu2024universally}, draw=brown]
            [GSR~\cite{in2024self}, draw=brown]
        ]
        [\textbf{Graph Injection Attack} \ref{sec:9.7.3}, draw=brown, top color=brown!40, bottom color=brown!40
            [HAO~\cite{chen2021understanding}, draw=brown]
        ]
    ]
    [\textbf{Urban Computing} \ref{sec:9.8}, draw=gray, top color=gray!10, bottom color=gray!10
        [SHGNN~\cite{xiao2023spatial}, draw=gray]
    ]
    [\textbf{Prompt Tuning} \ref{sec:9.9}, draw=pink, top color=pink!10, bottom color=pink!10
        [PGCL~\cite{gong2023prompt}, draw=pink]
        [SAP~\cite{ge2023enhancing}, draw=pink]
    ]
    [\textbf{Graph Coloring} \ref{sec:9.10}, draw=olive, top color=olive!10, bottom color=olive!10
        [AC-GNN~\cite{wang2024graph}, draw=olive]
    ]
    [\textbf{Binary Programming} \ref{sec:9.11}, draw=teal, top color=teal!10, bottom color=teal!10
        [BPGNN~\cite{eliasof2024graph}, draw=teal]
    ]
    [\textbf{Others} \ref{sec:9.12}, draw=lime, top color=lime!10, bottom color=lime!10
        [\textbf{Social Computing} \ref{sec:9.12.1}, draw=lime, top color=lime!20, bottom color=lime!20
            [\cite{gong2024towards}, draw=lime]
        ]
        [\textbf{Urban Dynamics} \ref{sec:9.12.2}, draw=lime, top color=lime!30, bottom color=lime!30
            [\cite{zheng2022graph}, draw=lime]
        ]
        [\textbf{Climate Change} \ref{sec:9.12.3}, draw=lime, top color=lime!40, bottom color=lime!40
            [\cite{bayraktar2023graph}, draw=lime]
        ]
        [\textbf{3D Geometry} \ref{sec:9.12.4}, draw=lime, top color=lime!50, bottom color=lime!50
            [\cite{bronstein2021geometric}, draw=lime]
        ]
        [\textbf{Graph Combinatorics} \ref{sec:9.12.5}, draw=lime, top color=lime!60, bottom color=lime!60 
            [\cite{wang2024graph}, draw=lime]
        ]
    ]
    ]
\end{forest}
}
\caption{Overview of heterophily-related applications. We only include a small portion of graph models for heterophily-related applications in this diagram, more models and details can be found in each section.}
\label{diag:application}
\end{figure*}

==> diagram_applications.tex <==
\begin{figure*}[ht!]
\centering
%\resizebox*{!}{\dimexpr\textheight-4\baselineskip\relax}{
\resizebox{1.0\textwidth}{!}{
\begin{forest}
    for tree={%
        my node,
        l sep+=5pt,
        grow'=east,
        edge={gray, thick},
        parent anchor=east,
        child anchor=west,
        if n children=0{tier=last}{},
        edge path={
            \noexpand\path [draw, \forestoption{edge}] (!u.parent anchor) -- +(10pt,0) |- (.child anchor)\forestoption{edge label};
        },
        if={isodd(n_children())}{
            for children={
                if={equal(n,(n_children("!u")+1)/2)}{calign with current}{}
            }
        }{}
    }
    [\textbf{Heterophily-Related Applications}, draw=black
    [\textbf{Fraud/Anomaly/Bot Detection} \ref{sec:9.1}, draw=green, top color=green!10, bottom color=green!10
        [\textbf{Fraud Detection} \ref{sec:9.1.1}, draw=green, top color=green!20, bottom color=green!20
            [\textbf{Neighborhood Partitioning and Grouping}, draw=green, top color=green!20, bottom color=green!20
                [H$^2$-FDetector~\cite{shi2022h2}, draw=green]
                [GAGA~\cite{wang2023label}, draw=green]
                [DRAG~\cite{kim2023dynamic}, draw=green]
            ]
            [\textbf{Spectral-Based Methods}, draw=green, top color=green!30, bottom color=green!30
                [SEC-GFD~\cite{xu2023revisiting}, draw=green]
                [SplitGNN~\cite{wu2023splitgnn}, draw=green]
            ]
        ]
        [\textbf{Anomaly Detection} \ref{sec:9.1.2}, draw=green, top color=green!30, bottom color=green!30
            [\textbf{Graph Structure Augmentation}, draw=green, top color=green!30, bottom color=green!30
                [GHRN~\cite{gao2023addressing}, draw=green]
                [SparseGAD~\cite{gong2023beyond}, draw=green]
                [HedGe~\cite{zhang2024generation}, draw=green]
            ]
            [\textbf{Metric-Guided Detection}, draw=green, top color=green!30, bottom color=green!30
                [TAM~\cite{qiao2024truncated}, draw=green]
            ]
            [\textbf{GAD-Specific Information Propagation}, draw=green, top color=green!30, bottom color=green!30
                [GDN~\cite{gao2023alleviating}, draw=green]
            ]
        ]
        [\textbf{Bot Detection} \ref{sec:9.1.3}, draw=green, top color=green!40, bottom color=green!40
            [BothH~\cite{li2023multi}, draw=green]
            [HOVER~\cite{ashmore2023hover}, draw=green]
            [HOFA~\cite{ye2023hofa}, draw=green]
        ]
    ]
    [\textbf{Generative Models} \ref{sec:9.2}, draw=red, top color=red!10, bottom color=red!10
        [\textbf{Molecule Generation} \ref{sec:9.2.1}, draw=red, top color=red!20, bottom color=red!20
            [HTFlows~\cite{wang2024molecule}, draw=red]
        ]
        [\textbf{Scene Graph Generation} \ref{sec:9.2.2}, draw=red, top color=red!30, bottom color=red!30
            [HL-Net~\cite{lin2022hl}, draw=red]
            [KWGNN~\cite{chen2024kumaraswamy}, draw=red]
        ]
    ]
    [\textbf{Classification and Clustering Tasks} \ref{sec:9.3}, draw=blue, top color=blue!10, bottom color=blue!10
        [\textbf{Link Prediction} \ref{sec:9.3.1}, draw=blue, top color=blue!20, bottom color=blue!20
            [DisenLink~\cite{zhou2022link}, draw=blue]
            [GRAFF-LP~\cite{di2023understanding}, draw=blue]
        ]
        [\textbf{Graph Classification} \ref{sec:9.3.2}, draw=blue, top color=blue!30, bottom color=blue!30
            [IHGNN~\cite{ye2022incorporating}, draw=blue]
            [MGS~\cite{ding2023self}, draw=blue]
        ]
        [\textbf{Graph Clustering} \ref{sec:9.3.3}, draw=blue, top color=blue!40, bottom color=blue!40
            [DGCN~\cite{pmlr-v202-pan23b}, draw=blue]
            [HoLe~\cite{gu2023homophily}, draw=blue]
            [AHGFC~\cite{wen2024homophily}, draw=blue]
        ]
    ]
    [\textbf{Recommender System} \ref{sec:9.4}, draw=yellow, top color=yellow!10, bottom color=yellow!10
        [SHaRe~\cite{jiang2024challenging}, draw=yellow]
    ]
    [\textbf{Biomedical} \ref{sec:9.5}, draw=violet, top color=violet!10, bottom color=violet!10
        [\textbf{Combination Therapy} \ref{sec:9.5.1}, draw=violet, top color=violet!20, bottom color=violet!20
            [DCMGCN~\cite{chen2022drug}, draw=violet]
        ]
        [\textbf{Drug Repositioning} \ref{sec:9.5.2}, draw=violet, top color=violet!30, bottom color=violet!30
            [SLGCN~\cite{liu2024slgcn}, draw=violet]
        ]
        [\textbf{Drug Discovery} \ref{sec:9.5.3}, draw=violet, top color=violet!40, bottom color=violet!40
            [HTFlows~\cite{ye2022incorporating}, draw=violet]
        ]
    ]
    [\textbf{Knowledge Distillation} \ref{sec:9.6}, draw=orange, top color=orange!10, bottom color=orange!10
        [SA-MLP~\cite{chen2022sa}, draw=orange]
        [VQGraph~\cite{yang2024vqgraph}, draw=orange]
    ]
    [\textbf{Adversarial Attack and Robustness} \ref{sec:9.7}, draw=brown, top color=brown!10, bottom color=brown!10
        [\textbf{Graph Structure Augmentation} \ref{sec:9.7.1}, draw=brown, top color=brown!20, bottom color=brown!20
            [GNNGUARD~\cite{zhang2020gnnguard}, draw=brown]
            [LP4GLN~\cite{cheng2023label}, draw=brown]
            [LHS~\cite{qiu2023refining}, draw=brown]
        ]
        [\textbf{Robust Graph Filter and Network Architecture} \ref{sec:9.7.2}, draw=brown, top color=brown!30, bottom color=brown!30
            [EvenNet~\cite{lei2022evennet}, draw=brown]
            [NSPGNN~\cite{zhu2024universally}, draw=brown]
            [GSR~\cite{in2024self}, draw=brown]
        ]
        [\textbf{Graph Injection Attack} \ref{sec:9.7.3}, draw=brown, top color=brown!40, bottom color=brown!40
            [HAO~\cite{chen2021understanding}, draw=brown]
        ]
    ]
    [\textbf{Urban Computing} \ref{sec:9.8}, draw=gray, top color=gray!10, bottom color=gray!10
        [SHGNN~\cite{xiao2023spatial}, draw=gray]
    ]
    [\textbf{Prompt Tuning} \ref{sec:9.9}, draw=pink, top color=pink!10, bottom color=pink!10
        [PGCL~\cite{gong2023prompt}, draw=pink]
        [SAP~\cite{ge2023enhancing}, draw=pink]
    ]
    [\textbf{Graph Coloring} \ref{sec:9.10}, draw=olive, top color=olive!10, bottom color=olive!10
        [AC-GNN~\cite{wang2024graph}, draw=olive]
    ]
    [\textbf{Binary Programming} \ref{sec:9.11}, draw=teal, top color=teal!10, bottom color=teal!10
        [BPGNN~\cite{eliasof2024graph}, draw=teal]
    ]
    [\textbf{Others} \ref{sec:9.12}, draw=lime, top color=lime!10, bottom color=lime!10
        [\textbf{Social Computing} \ref{sec:9.12.1}, draw=lime, top color=lime!20, bottom color=lime!20
            [\cite{gong2024towards}, draw=lime]
        ]
        [\textbf{Urban Dynamics} \ref{sec:9.12.2}, draw=lime, top color=lime!30, bottom color=lime!30
            [\cite{zheng2022graph}, draw=lime]
        ]
        [\textbf{Climate Change} \ref{sec:9.12.3}, draw=lime, top color=lime!40, bottom color=lime!40
            [\cite{bayraktar2023graph}, draw=lime]
        ]
        [\textbf{3D Geometry} \ref{sec:9.12.4}, draw=lime, top color=lime!50, bottom color=lime!50
            [\cite{bronstein2021geometric}, draw=lime]
        ]
        [\textbf{Graph Combinatorics} \ref{sec:9.12.5}, draw=lime, top color=lime!60, bottom color=lime!60 
            [\cite{wang2024graph}, draw=lime]
        ]
    ]
    ]
\end{forest}
}
\caption{Overview of heterophily-related applications. We only include a small portion of graph models for heterophily-related applications in this diagram, more models and details can be found in each section.}
\label{diag:application}
\end{figure*}

==> diagram_homogeneous.tex <==
\begin{figure*}[ht!]
\centering
\resizebox*{!}{\dimexpr\textheight-3.5\baselineskip\relax}{
\begin{forest}
    for tree={%
        my node,
        l sep+=5pt,
        grow'=east,
        edge={gray, thick},
        parent anchor=east,
        child anchor=west,
        if n children=0{tier=last}{},
        edge path={
            \noexpand\path [draw, \forestoption{edge}] (!u.parent anchor) -- +(10pt,0) |- (.child anchor)\forestoption{edge label};
        },
        if={isodd(n_children())}{
            for children={
                if={equal(n,(n_children("!u")+1)/2)}{calign with current}{}
            }
        }{}
    }
    [\textbf{GNNs for Heterophilic Homogeneous Graphs} \ref{sec:graph_models_for_heterophily}, draw=black
    [\textbf{Beyond Low-Pass Filter} \ref{sec:5.1}, draw=green, top color=green!10, bottom color=green!10
        [\textbf{Adaptive Combination of Low-pass and High-pass Filters} \ref{sec:5.1.1}, draw=green, top color=green!20, bottom color=green!20
            [GPRGNN~\cite{chien2021adaptive}, draw=green]
            %[FB-GNN~\cite{luan2022complete}, draw=green]
            [ACM-GNN~\cite{luan2022revisiting}, draw=green]
        ]
        [\textbf{Signed Message Passing} \ref{sec:5.1.2}, draw=green, top color=green!30, bottom color=green!30
            [FAGCN~\cite{bo2021beyond}, draw=green]
            [GloGNN~\cite{li2022finding}, draw=green]
            %[GGCN~\cite{yan2022two}, draw=green]
        ]
    ]
    [\textbf{Beyond Local Neighborhood Information} \ref{sec:5.2}, draw=red, top color=red!10, bottom color=red!10
        [\textbf{High-order Neighbor Mixing} \ref{sec:5.2.1}, draw=red, top color=red!20, bottom color=red!20
            [MixHop~\cite{abu2019mixhop}, draw=red]
            [H$_2$GCN~\cite{zhu2020beyond}, draw=red]
            %[UGCN~\cite{jin2021universal}, draw=red]
        ]
        [\textbf{Global Information from Latent Space} \ref{sec:5.2.2}, draw=red, top color=red!30, bottom color=red!30
            [Geom-GCN~\cite{pei2020geom}, draw=red]
            [NL-GNN~\cite{liu2021non}, draw=red]
            %[GPNN~\cite{yang2022graph}, draw=red]
        ]
        [\textbf{Path-based Aggregation} \ref{sec:5.2.3}, draw=red, top color=red!40, bottom color=red!40
            [PathNet~\cite{sun2022beyond}, draw=red]
            %[RAW-GNN~\cite{jin2022raw}, draw=red]
            [PathMLP~\cite{xie2023pathmlp}, draw=red]
        ]
    ]
    [\textbf{Advanced Network Architecture} \ref{sec:5.3}, draw=blue, top color=blue!10, bottom color=blue!10
        [\textbf{Physics-informed Graph Learning} \ref{sec:5.3.1}, draw=blue, top color=blue!20, bottom color=blue!20
            [ACMP~\cite{wang2022acmp}, draw=blue]
            [GREAD~\cite{choi2023gread}, draw=blue]
            %[CDE~\cite{zhao2023graph}, draw=blue]
        ]
        [\textbf{Expressive Spectral Filter} \ref{sec:5.3.2}, draw=blue, top color=blue!30, bottom color=blue!30
            [BernNet~\cite{he2021bernnet}, draw=blue]
            [UniFilter~\cite{li2023pc}, draw=blue]
            %[NFGNN~\cite{zheng2023node}, draw=blue]
        ]
        [\textbf{Similarity-guided Aggregation} \ref{sec:5.3.3}, draw=blue, top color=blue!40, bottom color=blue!40
            [UGCN~\cite{jin2021universal}, draw=blue]
            [SimP-GCN~\cite{jin2021node}, draw=blue]
            %[WRGNN~\cite{suresh2021breaking}, draw=blue]
        ]
        [\textbf{Enhanced Information Diffusion} \ref{sec:5.3.4}, draw=blue, top color=blue!50, bottom color=blue!50
            [SCN~\cite{bodnar2022neural}, draw=blue]
            %[LWGNN~\cite{dai2022label}, draw=blue]
            [Ordered GNN~\cite{song2023ordered}, draw=blue]
        ]
        [\textbf{Selective Message Propagation} \ref{sec:5.3.5}, draw=blue, top color=blue!60, bottom color=blue!60
            [DMP~\cite{yang2021diverse}, draw=blue]
            [FSGNN~\cite{maurya2022simplifying}, draw=blue]
            %[Gradient Gating~\cite{rusch2022gradient}, draw=blue]
        ]
        [\textbf{Compatibility Matrix Based Methods} \ref{sec:5.3.6}, draw=blue, top color=blue!70, bottom color=blue!70
            [CPGNN ~\cite{zhu2021graph}, draw=blue]
            [CLP~\cite{zhong2022simplifying}, draw=blue]
        ]
    ]
    [\textbf{Graph Structure Learning} \ref{sec:5.4}, draw=yellow, top color=yellow!10, bottom color=yellow!10
        [\textbf{Precomputed Graph Rewiring} \ref{sec:precomputed_graph_rewiring}, draw=yellow, top color=yellow!20, bottom color=yellow!20
            [\textbf{Homophily-oriented Rewiring}, draw=yellow, top color=yellow!20, bottom color=yellow!20
                [MVGFN~\cite{wang2023improving}, draw=yellow]
                [GOAL~\cite{zheng2023finding}, draw=yellow]
            ]
            [\textbf{Distance-oriented Rewiring}, draw=yellow, top color=yellow!20, bottom color=yellow!20
                [Adaptive Clustering~\cite{li2023restructuring}, draw=yellow]
                [DGAT~\cite{lu2024representation}, draw=yellow]
            ]
            [\textbf{Similarity-oriented Rewiring}, draw=yellow, top color=yellow!20, bottom color=yellow!20
                [ESC~\cite{jiang2021gcn}, draw=yellow]
                [DHGR~\cite{bi2022make}, draw=yellow]
                %[ECG~\cite{deac2023evolving}, draw=yellow]
            ]
            [\textbf{Information-theory Based Structure Learning}, draw=yellow, top color=yellow!20, bottom color=yellow!20
                [SE-GSL~\cite{zou2023se}, draw=yellow]
                [k-MIGNN~\cite{choi2023node}, draw=yellow]
            ]
            [\textbf{Others}, draw=yellow, top color=yellow!20, bottom color=yellow!20
                [LRGNN~\cite{liang2023predicting}, draw=yellow]
                [ALT~\cite{xu2023node}, draw=yellow]
                %[Free Labels~\cite{wu2023leveraging}, draw=yellow]
            ]
        ]
        [\textbf{End-to-end Structure Learning} \ref{sec:end_to_end_structure_learning}, draw=yellow, top color=yellow!30, bottom color=yellow!30
            [\textbf{Probabilistic Methods}, draw=yellow, top color=yellow!30, bottom color=yellow!30
                [GEN~\cite{wang2021graph}, draw=yellow]
                [L2A~\cite{wu2023learning}, draw=yellow]
            ]
            [\textbf{Edge Prediction}, draw=yellow, top color=yellow!30, bottom color=yellow!30
                [GAUG~\cite{zhao2021data}, draw=yellow]
                [SGAT~\cite{ye2021sparse}, draw=yellow]
            ]
            [\textbf{Similarity-guided Connection}, draw=yellow, top color=yellow!30, bottom color=yellow!30
                [ConSM~\cite{choi2022finding}, draw=yellow]
                [GNN-SATA~\cite{yang2024graph}, draw=yellow]
            ]
            [\textbf{Edge Weight Refinement}, draw=yellow, top color=yellow!30, bottom color=yellow!30
                [GGCN~\cite{yan2022two}, draw=yellow]
            ]
        ]
    ]
    [\textbf{Graph Transformers} \ref{sec:5.5}, draw=orange, top color=orange!10, bottom color=orange!10
        [\textbf{Signed Self-attention}, draw=orange, top color=orange!20, bottom color=orange!20
            [SignGT~\cite{chen2023signgt}, draw=orange]
            [SADE-GCN~\cite{lai2023self}, draw=orange]
        ]
        [\textbf{Virtual Nodes and Connections}, draw=orange, top color=orange!30, bottom color=orange!30
            [GOAT~\cite{kong2023goat}, draw=orange]
            [VCR-Graphormer~\cite{fu2024vcrgraphormer}, draw=orange]
        ]
        [\textbf{Pooling and Coarsening}, draw=orange, top color=orange!40, bottom color=orange!40
            [ANS-GT~\cite{zhang2022hierarchical}, draw=orange]
            [Gapformer~\cite{liu2023gapformer}, draw=orange]
        ]
        [\textbf{Positional/Structural Encoding}, draw=orange, top color=orange!50, bottom color=orange!50
            [DGT~\cite{park2022deformable}, draw=orange]
            [MPformer~\cite{2024mpformer}, draw=orange]
        ]
        [\textbf{Heterophily-Specific Graph Transformer}, draw=orange, top color=orange!60, bottom color=orange!60
            [HL-Net~\cite{lin2022hl}, draw=orange]
            [HGAT~\cite{wang2023heterophily}, draw=orange]
        ]
    ]
    [\textbf{Others} \ref{sec:5.6}, draw=brown, top color=brown!10, bottom color=brown!10
        [\textbf{Neural Architecture Search} \ref{sec:5.6.1}, draw=brown, top color=brown!20, bottom color=brown!20
            [LADDER-GNN~\cite{zeng2021relational}, draw=brown]
            %[IIE-GNN~\cite{wei2022enhancing}, draw=brown]
            [F2GNN~\cite{wei2022designing}, draw=brown]
        ]
        [\textbf{Edge Directionality} \ref{sec:5.6.2}, draw=brown, top color=brown!30, bottom color=brown!30
            [Dir-GNN~\cite{rossi2023edge}, draw=brown]
            %[AMUD~\cite{sun2023breaking}, draw=brown]
            [HoloNets~\cite{koke2023holonets}, draw=brown]
        ]
        [\textbf{Graph Mamba} \ref{sec:5.6.3}, draw=brown, top color=brown!40, bottom color=brown!40
            [GMN~\cite{behrouz2024graph}, draw=brown]
        ]
        [\textbf{Memory-based Method} \ref{sec:5.6.4}, draw=brown, top color=brown!50, bottom color=brown!50
            %[MMP~\cite{chen2022memory}, draw=brown]
            [HP-GMN~\cite{xu2022hp}, draw=brown]
            [DisamGCL~\cite{zhao2024disambiguated}, draw=brown]
        ]
        [\textbf{Remaining Methods} \ref{sec:5.6.5}, draw=brown, top color=brown!60, bottom color=brown!60
            [\textbf{Graph Capsule Network}, draw=brown, top color=brown!60, bottom color=brown!60
                [NCGNN~\cite{yang2022ncgnn}, draw=brown]
            ]
            [\textbf{Relation Encoder}, draw=brown, top color=brown!60, bottom color=brown!60
                [VR-GNN~\cite{shi2022vr}, draw=brown]
                [RFA-GNN~\cite{wu2023beyond}, draw=brown]
            ]
            [\textbf{Deep Reinforcement Learning}, draw=brown, top color=brown!60, bottom color=brown!60
                [GraphRARE~\cite{peng2023graphrare}, draw=brown]
            ]
            [\textbf{Uncertainty-aware Model}, draw=brown, top color=brown!60, bottom color=brown!60
                [Uncertainty Debiasing~\cite{liu2022ud}, draw=brown]
            ]
            [\textbf{Adaptive Mixture of Multiple Modules}, draw=brown, top color=brown!60, bottom color=brown!60
                [MWGNN~\cite{ma2022meta}, draw=brown]
                [CAGNN~\cite{chen2023exploiting}, draw=brown]
            ]
            [\textbf{Masking}, draw=brown, top color=brown!60, bottom color=brown!60
                [GraphTU~\cite{gao2023topology}, draw=brown]
            ]
        ]
    ]
    ]
\end{forest}
}
\caption{Overview of graph models for homogeneous graphs with heterophily. We only include a small portion of graph models on homogeneous graphs in this diagram, more models and details can be found in each section.}
\label{diag:homo}
\end{figure*}

==> diagram_homogeneous_graphs.tex <==
\newcolumntype{C}[1]{>{\centering}p{#1}}

\begin{figure*}
\centering
\resizebox{1\hsize}{!}{
\begin{forest}
for tree={
  font=\footnotesize,
  if level=0{align=center}
  {% allow multi-line text and set alignment
    align={@{}C{60mm}@{}}, % <---only changed this
  },
  grow=east,
  %font=\sffamily\bfseries,
  edge path={
    \noexpand\path [draw, \forestoption{edge}] (!u.parent anchor) -- +(4mm,0) |- (.child anchor)\forestoption{edge label};
  },
  parent anchor=east,
  child anchor=west,
  s sep = -3mm, %vertical space between nodes
  l sep=6mm,  % horizontal space between nodes
  inner sep = 3mm, %node size
  %l sep=10mm,
  tier/.wrap pgfmath arg={tier #1}{level()},
  edge={thick, rounded corners=2pt},
}
[Models
  [Beyond Low-pass Filter
    [Adaptive Combination of Low-pass and High-pass Filters]
    [Signed Message Passing]
  ]
  [Beyond Local Neighborhood Information
    [High-order Neighbor Mixing]
    [Global Information from Latent Space]
    [Path-based Aggregation]]
  [Advanced Network Architectures
    [Physics (PDE)-informed Diffusion Process]
    [Expressive Spectral Filter]
    [Similarity-guided Aggregation]
    [Selective Information Propagation]
    [Heterophily-Specific Message Passing]
    [Compatability Matrix Based Methods]
    ]
   [Graph Structure Learning
    [Precomputed Graph Rewiring
     [Similarity-oriented Rewiring]
     [Homophily-oriented Rewiring]
     [Distance-oriented Rewiring]
     [Information-theory Based Structure Learning]
     [Others]]
    [End-to-end Structure Learning
     [Probabilistic Methods]
     [Similarity-guided Connection]
     [Edge Weight Refinement]]
   ]
   [Graph Transformers
    [Signed Self-attention]
    [Virtual Nodes and Connections]
    [Pooling and Coarsening]
    [Positional/Structural Encoding]
    [Heterophily-Specific Graph Transformer]]
    [Others, draw
     [Neural Architecture Search]
     [Edge Directionality]
     [Graph Mamba]
     [Memory-based Method]
     [Remaining Methods
      [Graph Capsule Network]
      [Relation Encoder]
      [Deep Reinforcement Learning]
      [Uncertainty-aware Model]
      [Adaptive Mixture of Multiple Modules]
      [Masking]
      ]
      ]
  ]
]
\end{forest}
}
\caption{Graph models on homogeneous graphs}
\label{diagram:homogeneous_graphs}
\end{figure*}


==> homogeneous.tex <==
\begin{figure*}[ht!]
\centering
\resizebox*{!}{\dimexpr\textheight-4\baselineskip\relax}{
\begin{forest}
    for tree={%
        my node,
        l sep+=5pt,
        grow'=east,
        edge={gray, thick},
        parent anchor=east,
        child anchor=west,
        if n children=0{tier=last}{},
        edge path={
            \noexpand\path [draw, \forestoption{edge}] (!u.parent anchor) -- +(10pt,0) |- (.child anchor)\forestoption{edge label};
        },
        if={isodd(n_children())}{
            for children={
                if={equal(n,(n_children("!u")+1)/2)}{calign with current}{}
            }
        }{}
    }
    [\textbf{GNNs for Heterophilic Homogeneous Graphs}, draw=black
    [\textbf{Beyond Low-Pass Filter} \ref{sec:5.1}, draw=green, top color=green!10, bottom color=green!10
        [\textbf{Adaptive Combination of Low-pass and High-pass Filters} \ref{sec:5.1.1}, draw=green, top color=green!20, bottom color=green!20
            [GPRGNN~\cite{chien2021adaptive}, draw=green]
            [FB-GNN~\cite{luan2022complete}, draw=green]
            [ACM-GNN~\cite{luan2022revisiting}, draw=green]
        ]
        [\textbf{Signed Message Passing} \ref{sec:5.1.2}, draw=green, top color=green!30, bottom color=green!30
            [FAGCN~\cite{bo2021beyond}, draw=green]
            [GloGNN~\cite{li2022finding}, draw=green]
            [GGCN~\cite{yan2022two}, draw=green]
        ]
    ]
    [\textbf{Beyond Local Neighborhood Information} \ref{sec:5.2}, draw=red, top color=red!10, bottom color=red!10
        [\textbf{High-order Neighbor Mixing} \ref{sec:5.2.1}, draw=red, top color=red!20, bottom color=red!20
            [MixHop~\cite{abu2019mixhop}, draw=red]
            [H$_2$GCN~\cite{zhu2020beyond}, draw=red]
            [UGCN~\cite{jin2021universal}, draw=red]
        ]
        [\textbf{Global Information from Latent Space} \ref{sec:5.2.2}, draw=red, top color=red!30, bottom color=red!30
            [Geom-GCN~\cite{pei2020geom}, draw=red]
            [NL-GNN~\cite{liu2021non}, draw=red]
            [GPNN~\cite{yang2022graph}, draw=red]
        ]
        [\textbf{Path-based Aggregation} \ref{sec:5.2.3}, draw=red, top color=red!40, bottom color=red!40
            [PathNet~\cite{sun2022beyond}, draw=red]
            [RAW-GNN~\cite{jin2022raw}, draw=red]
            [PathMLP~\cite{xie2023pathmlp}, draw=red]
        ]
    ]
    [\textbf{Advanced Network Architecture} \ref{sec:5.3}, draw=blue, top color=blue!10, bottom color=blue!10
        [\textbf{Physics-informed Graph Learning} \ref{sec:5.3.1}, draw=blue, top color=blue!20, bottom color=blue!20
            [ACMP~\cite{wang2022acmp}, draw=blue]
            [GREAD~\cite{choi2023gread}, draw=blue]
            [CDE~\cite{zhao2023graph}, draw=blue]
        ]
        [\textbf{Expressive Spectral Filter} \ref{sec:5.3.2}, draw=blue, top color=blue!30, bottom color=blue!30
            [BernNet~\cite{he2021bernnet}, draw=blue]
            [UniFilter~\cite{li2023pc}, draw=blue]
            [NFGNN~\cite{zheng2023node}, draw=blue]
        ]
        [\textbf{Similarity-guided Aggregation} \ref{sec:5.3.3}, draw=blue, top color=blue!40, bottom color=blue!40
            [UGCN~\cite{jin2021universal}, draw=blue]
            [SimP-GCN~\cite{jin2021node}, draw=blue]
            [WRGNN~\cite{suresh2021breaking}, draw=blue]
        ]
        [\textbf{Enhanced Information Diffusion} \ref{sec:5.3.4}, draw=blue, top color=blue!50, bottom color=blue!50
            [SCN~\cite{bodnar2022neural}, draw=blue]
            [LWGNN~\cite{dai2022label}, draw=blue]
            [Ordered GNN~\cite{song2023ordered}, draw=blue]
        ]
        [\textbf{Selective Message Propagation} \ref{sec:5.3.5}, draw=blue, top color=blue!60, bottom color=blue!60
            [DMP~\cite{yang2021diverse}, draw=blue]
            [FSGNN~\cite{maurya2022simplifying}, draw=blue]
            [Gradient Gating~\cite{rusch2022gradient}, draw=blue]
        ]
        [\textbf{Compatibility Matrix Based Methods} \ref{sec:5.3.6}, draw=blue, top color=blue!70, bottom color=blue!70
            [CPGNN ~\cite{zhu2021graph}, draw=blue]
            [CLP~\cite{zhong2022simplifying}, draw=blue]
        ]
    ]
    [\textbf{Graph Structure Learning} \ref{sec:5.4}, draw=yellow, top color=yellow!10, bottom color=yellow!10
        [\textbf{Precomputed Graph Rewiring} \ref{sec:5.4.1}, draw=yellow, top color=yellow!20, bottom color=yellow!20
            [\textbf{Homophily-oriented Rewiring}, draw=yellow, top color=yellow!20, bottom color=yellow!20
                [MVGFN~\cite{wang2023improving}, draw=yellow]
                [GOAL~\cite{zheng2023finding}, draw=yellow]
            ]
            [\textbf{Distance-oriented Rewiring}, draw=yellow, top color=yellow!20, bottom color=yellow!20
                [Adaptive Clustering~\cite{li2023restructuring}, draw=yellow]
                [DGAT~\cite{lu2024representation}, draw=yellow]
            ]
            [\textbf{Similarity-oriented Rewiring}, draw=yellow, top color=yellow!20, bottom color=yellow!20
                [ESC~\cite{jiang2021gcn}, draw=yellow]
                [DHGR~\cite{bi2022make}, draw=yellow]
                [ECG~\cite{deac2023evolving}, draw=yellow]
            ]
            [\textbf{Information-theory Based Structure Learning}, draw=yellow, top color=yellow!20, bottom color=yellow!20
                [SE-GSL~\cite{zou2023se}, draw=yellow]
                [k-MIGNN~\cite{choi2023node}, draw=yellow]
            ]
            [\textbf{Others}, draw=yellow, top color=yellow!20, bottom color=yellow!20
                [LRGNN~\cite{liang2023predicting}, draw=yellow]
                [ALT~\cite{xu2023node}, draw=yellow]
                [Free Labels~\cite{wu2023leveraging}, draw=yellow]
            ]
        ]
        [\textbf{End-to-end Structure Learning} \ref{sec:5.4.2}, draw=yellow, top color=yellow!30, bottom color=yellow!30
            [\textbf{Probabilistic Methods}, draw=yellow, top color=yellow!30, bottom color=yellow!30
                [GEN~\cite{wang2021graph}, draw=yellow]
                [L2A~\cite{wu2023learning}, draw=yellow]
            ]
            [\textbf{Edge Prediction}, draw=yellow, top color=yellow!30, bottom color=yellow!30
                [GAUG~\cite{zhao2021data}, draw=yellow]
                [SGAT~\cite{ye2021sparse}, draw=yellow]
            ]
            [\textbf{Similarity-guided Connection}, draw=yellow, top color=yellow!30, bottom color=yellow!30
                [ConSM~\cite{choi2022finding}, draw=yellow]
                [GNN-SATA~\cite{yang2024graph}, draw=yellow]
            ]
            [\textbf{Edge Weight Refinement}, draw=yellow, top color=yellow!30, bottom color=yellow!30
                [GGCN~\cite{yan2022two}, draw=yellow]
            ]
        ]
    ]
    [\textbf{Graph Transformers} \ref{sec:5.5}, draw=orange, top color=orange!10, bottom color=orange!10
        [\textbf{Signed Self-attention}, draw=orange, top color=orange!20, bottom color=orange!20
            [SignGT~\cite{chen2023signgt}, draw=orange]
            [SADE-GCN~\cite{lai2023self}, draw=orange]
        ]
        [\textbf{Virtual Nodes and Connections}, draw=orange, top color=orange!30, bottom color=orange!30
            [GOAT~\cite{kong2023goat}, draw=orange]
            [VCR-Graphormer~\cite{fu2024vcrgraphormer}, draw=orange]
        ]
        [\textbf{Pooling and Coarsening}, draw=orange, top color=orange!40, bottom color=orange!40
            [ANS-GT~\cite{zhang2022hierarchical}, draw=orange]
            [Gapformer~\cite{liu2023gapformer}, draw=orange]
        ]
        [\textbf{Positional/Structural Encoding}, draw=orange, top color=orange!50, bottom color=orange!50
            [DGT~\cite{park2022deformable}, draw=orange]
            [MPformer~\cite{2024mpformer}, draw=orange]
        ]
        [\textbf{Heterophily-Specific Graph Transformer}, draw=orange, top color=orange!60, bottom color=orange!60
            [HL-Net~\cite{lin2022hl}, draw=orange]
            [HGAT~\cite{wang2023heterophily}, draw=orange]
        ]
    ]
    [\textbf{Others} \ref{sec:5.6}, draw=brown, top color=brown!10, bottom color=brown!10
        [\textbf{Neural Architecture Search} \ref{sec:5.6.1}, draw=brown, top color=brown!20, bottom color=brown!20
            [LADDER-GNN~\cite{zeng2021relational}, draw=brown]
            [IIE-GNN~\cite{wei2022enhancing}, draw=brown]
            [F2GNN~\cite{wei2022designing}, draw=brown]
        ]
        [\textbf{Edge Directionality} \ref{sec:5.6.2}, draw=brown, top color=brown!30, bottom color=brown!30
            [Dir-GNN~\cite{rossi2023edge}, draw=brown]
            [AMUD~\cite{sun2023breaking}, draw=brown]
            [HoloNets~\cite{koke2023holonets}, draw=brown]
        ]
        [\textbf{Graph Mamba} \ref{sec:5.6.3}, draw=brown, top color=brown!40, bottom color=brown!40
            [GMN~\cite{behrouz2024graph}, draw=brown]
        ]
        [\textbf{Memory-based Method} \ref{sec:5.6.4}, draw=brown, top color=brown!50, bottom color=brown!50
            [MMP~\cite{chen2022memory}, draw=brown]
            [HP-GMN~\cite{xu2022hp}, draw=brown]
            [DisamGCL~\cite{zhao2024disambiguated}, draw=brown]
        ]
        [\textbf{Remaining Methods} \ref{sec:5.6.5}, draw=brown, top color=brown!60, bottom color=brown!60
            [\textbf{Graph Capsule Network}, draw=brown, top color=brown!60, bottom color=brown!60
                [NCGNN~\cite{yang2022ncgnn}, draw=brown]
            ]
            [\textbf{Relation Encoder}, draw=brown, top color=brown!60, bottom color=brown!60
                [VR-GNN~\cite{shi2022vr}, draw=brown]
                [RFA-GNN~\cite{wu2023beyond}, draw=brown]
            ]
            [\textbf{Deep Reinforcement Learning}, draw=brown, top color=brown!60, bottom color=brown!60
                [GraphRARE~\cite{peng2023graphrare}, draw=brown]
            ]
            [\textbf{Uncertainty-aware Model}, draw=brown, top color=brown!60, bottom color=brown!60
                [Uncertainty Debiasing~\cite{liu2022ud}, draw=brown]
            ]
            [\textbf{Adaptive Mixture of Multiple Modules}, draw=brown, top color=brown!60, bottom color=brown!60
                [MWGNN~\cite{ma2022meta}, draw=brown]
                [CAGNN~\cite{chen2023exploiting}, draw=brown]
            ]
            [\textbf{Masking}, draw=brown, top color=brown!60, bottom color=brown!60
                [GraphTU~\cite{gao2023topology}, draw=brown]
            ]
        ]
    ]
    ]
\end{forest}
}
\caption{Overview of graph models for homogeneous graphs with heterophily. We only include a small portion of graph models on homogeneous graphs in this diagram, more models and details can be found in each section.}
\label{diag:homo}
\end{figure*}

==> tab_statistics_datasets.tex <==
% Table generated by Excel2LaTeX from sheet 'homogeneous'
\begin{table}[htbp]
  \centering
  \caption{Statistics of Datasets}
   \resizebox{1\hsize}{!}{
    \begin{tabular}{c|cccccc}
    \toprule
    \toprule
    \multicolumn{1}{c|}{} & \multicolumn{1}{p{3.855em}}{\#nodes} & \multicolumn{1}{p{4.715em}}{\#edges} & \multicolumn{1}{p{3.855em}}{\#feature} & \multicolumn{1}{p{3.715em}}{\#classes} & \multicolumn{1}{p{4.93em}}{edge homo} & \multicolumn{1}{p{5em}}{node homo} \\
    \midrule
    Cornell & 183   & 295   & 1,703 & 5     & 0.5669 & 0.3855 \\
    Wisconsin & 251   & 499   & 1,703 & 5     & 0.4480 & 0.1498 \\
    Texas & 183   & 309   & 1,703 & 5     & 0.4106 & 0.0968 \\
    Film  & 7,600 & 33,544 & 931   & 5     & 0.3750 & 0.2210 \\
    Chameleon & 2,277 & 36,101 & 2,325 & 5     & 0.2795 & 0.2470 \\
    Squirrel & 5,201 & 217,073 & 2,089 & 5     & 0.2416 & 0.2156 \\
    Deezer-Europe & 28,281 & 92,752 & 31,241 & 2     & 0.5251 & 0.5299 \\
    Cora  & 2,708 & 5,429 & 1,433 & 7     & 0.8100 & 0.8252 \\
    CiteSeer & 3,327 & 4,732 & 3,703 & 6     & 0.7362 & 0.7175 \\
    PubMed & 19,717 & 44,338 & 500   & 3     & 0.8024 & 0.7924 \\
    Penn94 & 41,554 & 1,362,229 & 5     & 2     & 0.47  & 0.483 \\
    arxiv-year & 169,343 & 1,166,243 & 128   & 5     & 0.222 & 0.289 \\
    genius & 421,961 & 984,979 & 12    & 2     & 0.618 & 0.508 \\
    twitch-gamer & 168,114 & 6,797,557 & 7     & 2     & 0.545 & 0.556 \\
    \bottomrule
    \bottomrule
    \end{tabular}%
    }
  \label{tab:datasets_stats}%
\end{table}%

